MFTCoder: Boosting Code LLMs with Multitask Fine-Tuning

Code LLMs have emerged as a specialized research field, with remarkable studies dedicated to enhancing model's coding capabilities through fine-tuning on pre-trained models. Previous fine-tuning approaches were typically tailored to specific downstream tasks or scenarios, which meant separate fine-tuning for each task, requiring extensive training resources and posing challenges in terms of deployment and maintenance. Furthermore, these approaches failed to leverage the inherent interconnectedness among different code-related tasks. To overcome these limitations, we present a multi-task fine-tuning framework, MFTcoder, that enables simultaneous and parallel fine-tuning on multiple tasks. By incorporating various loss functions, we effectively address common challenges in multi-task learning, such as data imbalance, varying difficulty levels, and inconsistent convergence speeds. Extensive experiments have conclusively demonstrated that our multi-task fine-tuning approach outperforms both individual fine-tuning on single tasks and fine-tuning on a mixed ensemble of tasks. Moreover, MFTcoder offers efficient training capabilities, including efficient data tokenization modes and PEFT fine-tuning, resulting in significantly improved speed compared to traditional fine-tuning methods. MFTcoder seamlessly integrates with several mainstream open-source LLMs, such as CodeLLama and Qwen. Leveraging the CodeLLama foundation, our MFTcoder fine-tuned model, \textsc{CodeFuse-CodeLLama-34B}, achieves an impressive pass@1 score of 74.4\% on the HumaneEval benchmark, surpassing GPT-4 performance (67\%, zero-shot). MFTCoder is open-sourced at \url{https://github.com/codefuse-ai/MFTCOder}

==> data.tex <==
\section{Data}

This is the data section ...

==> related.tex <==
\section{Related Work}

\subsubsection{\textbf{Large Language Models}}

The capabilities demonstrated by GPT-3.5~\cite{brown2020language, ouyang2022training} and GPT-4~\cite{openai2023gpt4} have shown the potential of large language models (LLMs) based on the Transformer~\cite{vaswani2023attention} architecture, with billions or even trillions of parameters, in the journey towards achieving general artificial intelligence. This has quickly sparked a research and development frenzy, leading to the successive release of a wave of LLMs. 
Google unveiled its Bard product powered by PaLM~\cite{chowdhery2022palm} and PaLM 2~\cite{anil2023palm}, Anthropic introduced Claude 2~\cite{anthropic2023claude}, Baidu launched ERNIE Bot~\cite{xu2022long}, and DeepMind presented Chinchilla~\cite{hoffmann2022training}.
In addition to these proprietary models, there has been a constant stream of open-source general LLMs as well. Notable examples include BLOOM~\cite{scao2022bloom} by BigScience, OPT~\cite{zhang2022opt} and LLama 1/2~\cite{touvron2023llama, touvron2023llama2} by Meta,  Qwen~\cite{qwen} by Alibaba, CodeFuse~\cite{di2023codefuse13b} by AntGroup, Baichuan 1/2~\cite{baichuan2023baichuan2}by Baichuan AI, ChatGLM 1/2~\cite{zeng2022glm, du2022glm} by Tsinghua University, and Falcon~\cite{falcon40b} by TII. These endeavors have democratized LLM research, making it no longer exclusive to large corporations and accelerating advancements in the field.





\subsubsection{\textbf{Large Language Models for Code}}

It was observed that including code data in the training data for LLMs such as GPT-J~\cite{wang2021gpt} and GPT-Neo~\cite{black2021gpt} could enhance their ability to understand and generate code. Currently, incorporating code data in the training data has become a standard practice for training general-purpose LLMs, and code competency testing has become an essential component of evaluating LLMs across various dimensions. Both closed-source and open-source LLMs mentioned earlier adhere to this approach. Additionally, there are specialized pre-trained and fine-tuned LLMs designed specifically for code-related tasks. 

CodeX~\cite{chen2021codex}, fine-tuned on public code repositories from GitHub, represents a significant milestone in LLMs for code, and its variant powers GitHub Copilot~\footnote{https://github.com/features/copilot}, transforming the landscape of code generation.
% 随后，PolyCoder~\cite{xu2022systematic}、InCoder~\cite{fried2023incoder}、CodeGen~\cite{nijkamp2022codegen}、PaLM-Coder~\cite{chowdhery2022palm}、GPT-Neox、PanGu-Coder~\cite{christopoulou2022pangucoder}、Santa Coder~\cite{allal2023santacoder}、CodeGeeX等代码专用LLMs相继发布。
Subsequently, specialized code-oriented LLMs such as PolyCoder~\cite{xu2022systematic}, InCoder~\cite{fried2023incoder}, CodeGen~\cite{nijkamp2022codegen}, PaLM-Coder~\cite{chowdhery2022palm}, GPT-Neox~\cite{black2022gptneox20b}, PanGu-Coder~\cite{christopoulou2022pangucoder}, Santa Coder~\cite{allal2023santacoder}, and CodeGeeX~\cite{zheng2023codegeex} emerged successively.
A significant milestone that followed was the release of StarCoder~\cite{li2023starcoder} by the BigCode, an open-source model that achieved performance on par with the OpenAI code-cushman-001 model (a version of CodeX~\cite{chen2021codex}) in terms of code proficiency. Building upon StarCoder, the fine-tuned models WizardCoder-15B~\cite{luo2023wizardcoder} and Pangu-Coder 2~\cite{shen2023pangu}, both open-source models, surpassed GPT-3.5 on the HumaneEval~\cite{chen2021codex} benchmark for the first time. The former highlighted and validated the effectiveness of the Evol-Instruct~\cite{xu2023wizardlm} method in Code LLMs, while the latter emphasized and validated the effectiveness of the RRTF (Rank Responses to align Test\&Teacher Feedback) method. Another groundbreaking achievement was the development of the CodeLLama series of models by Meta~\cite{roziere2023code}, which were further trained on LLama 2~\cite{touvron2023llama2}. Fine-tuned models such as WizardCoder-34B and Phind-CodeLlama, based on CodeLLama-34B-Python, surpassed GPT-4 in HumanEval.
n addition, PHI 1~\cite{gunasekar2023textbooks} and 1.5~\cite{textbooks2} proposed the use of high-quality training data to enable even small models to achieve code proficiency on par with larger models.
OctoPack~\cite{muennighoff2023octopack} showcased the effectiveness of utilizing Git commit data for fine-tuning Code LLMs.



\subsubsection{\textbf{Multi-task Learning}}

Google introduced T5~\cite{raffel2023exploring}, where they explored the application of MTL techniques. However, their approach was relatively straightforward. They simply mixed the data from all tasks together in different proportions for fine-tuning and proposed several methods for data blending. 
Meta further introduced Mupper~\cite{aghajanyan2021muppet}, which applies multi-task learning between pretraining and fine-tuning, termed as pre-fine-tuning (PFT). They discovered that incorporating this step enhances the performance of the pretrained model across various downstream tasks and significantly improves the speed of fine-tuning. However, if the number of tasks in PFT is too small, it can have a negative impact on the model's performance. Therefore, it is recommended to have a minimum of 15 tasks for optimal results.
Building upon T5, Google introduced ExT5~\cite{aribandi2022ext5}, which increased the number of tasks to 107. They found that as long as the number of tasks in pretraining is sufficiently large, even if there may be mutual interference among tasks, the ultimate results are still remarkably good. Ultimately, ExT5 outperformed T5 across multiple metrics.

